More Effective Crossover Operators for the All-Pairs Shortest Path Problem

The all-pairs shortest path problem is the first non-artificial problem for which it was shown that adding crossover can significantly speed up a mutation-only evolutionary algorithm. Recently, the analysis of this algorithm was refined and it was shown to have an expected optimization time (w.r.t. the number of fitness evaluations) of $\Theta(n^{3.25}(\log n)^{0.25})$. In contrast to this simple algorithm, evolutionary algorithms used in practice usually employ refined recombination strategies in order to avoid the creation of infeasible offspring. We study extensions of the basic algorithm by two such concepts which are central in recombination, namely \emph{repair mechanisms} and \emph{parent selection}. We show that repairing infeasible offspring leads to an improved expected optimization time of $\mathord{O}(n^{3.2}(\log n)^{0.2})$. As a second part of our study we prove that choosing parents that guarantee feasible offspring results in an even better optimization time of $\mathord{O}(n^{3}\log n)$. Both results show that already simple adjustments of the recombination operator can asymptotically improve the runtime of evolutionary algorithms.

==> conclusions.tex <==

We have shown how the use of repair mechanisms or appropriate selection strategies can speed up crossover-based evolutionary algorithms for the \AllPairs problem (and some other problems with a similar structure). 
However, it remains a challenge to understand the usefulness of crossover in evolutionary computation in a rigorous way for other combinatorial optimization problems.

The evolutionary algorithm examined for the APSP problem makes use of a strong diversity mechanism (each individual represents a path between a different pair of vertices) that allows to show the usefulness of crossover. Often evolutionary algorithms use much weaker diversity mechanism such as niching, deterministic crowding and fitness sharing and the goal is to compute just a single solution instead of a set of solutions. We state it as an open problem to show that crossover speeds up evolutionary algorithms for single-objective combinatorial optimization using one of the stated diversity mechanisms. 

On the other hand, multi-objective problems use in a natural way a diversity mechanisms according to Pareto dominance. Often the population of an evolutionary algorithm for multi-objective optimization contains a population which represents the different tradeoffs with respect to the given objective function at a certain time step. It would be interesting to have rigorous results that show the usefulness of crossover in evolutionary multi-objective optimization.


==> definespreprint.tex <==
% $Date: 2008-02-01 19:00:20 +0100 (Fri, 01 Feb 2008) $
% $Revision: 155 $
% $Author: cklein $
\usepackage{amsthm}
\usepackage{exscale}
\usepackage{setspace}
\usepackage{a4wide}

%\usepackage[obey]{fixacm}
\usepackage{amsmath,amssymb}
\usepackage{color}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{url}
%\usepackage{dsfont}
\usepackage{subfigure}
\usepackage{nicefrac}
\usepackage{tikz}
\usetikzlibrary{decorations,arrows}
\usetikzlibrary{decorations.pathmorphing}
\usepgflibrary{decorations.pathreplacing} 

\graphicspath{{figs/}}

\usepackage[algo2e,lined,vlined,linesnumbered]{algorithm2e}
\SetKwFor{Function}{function}{is}{end function}
\newcommand{\assign}{\leftarrow}
\SetAlgoCaptionLayout{small}

% Comments, Margins, etc
\newcommand{\ignore}[1]{}
\newcommand{\fixme}[1]{\textcolor{red}{\textbf{ FIXME }[#1]}}
\newcommand{\merk}[1]{{\textcolor{red}{\bf #1}}}
\newcommand{\eg}{e.\,g.\xspace}
% Theorem environment


% Mathematic abbreviations
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Prob}{\ensuremath{\mathrm{Prob}}}
\newcommand{\PR}[1]{\Prob\left[#1\right]}
\newcommand{\EXP}{\ensuremath{\operatorname{E}}}
\newcommand{\E}[1]{\EXP\left[#1\right]}
\newcommand{\Hm}[1][m]{\ensuremath{{\mathcal H}_#1}} %% Harmonic number
\newcommand{\Po}{\ensuremath{\mathop{\rm Pois}}}
\newcommand{\Ber}{\ensuremath{\mathop{\rm Ber}}}
\newcommand{\I}{\ensuremath{I}}

\newcommand{\XCal}{{\cal X}}
\newcommand{\opt}{\text{opt}}
\newcommand{\euler}{\mathrm{e}}


\newcommand{\bigo}[1]{\mathord{O}\mathord{\left(#1\right)}}
\newcommand{\littleo}[1]{\mathord{o}\mathord{\left(#1\right)}}
\newcommand{\bigomega}[1]{\mathord{\Omega}\mathord{\left(#1\right)}}
\newcommand{\littleomega}[1]{\mathord{\omega}\mathord{\left(#1\right)}}
\newcommand{\bigtheta}[1]{\mathord{\Theta}\mathord{\left(#1\right)}}
\newcommand{\ee}{\varepsilon}
\newcommand{\ie}{i.~e.\xspace}
\newcommand{\wrt}{w.~r.~t.\xspace}
\newcommand{\whp}{w.\,h.\,p.\xspace}
\newcommand{\uar}{u.~a.~r.\xspace}
\newcommand{\vl}{V_{\ell}^{2}}
\newcommand{\vk}{V_{k}^{2}}
\newcommand{\SSGA}{Steady State GA$_{\text{APSP}}$\xspace}
\newcommand{\PCal}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\AllPairs}{all-pairs shortest path\xspace}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}

%\newtheorem{proof}{Proof}
\renewcommand{\endproof}{\qed}
\newcommand{\com}[1]{\marginpar{\scriptsize\raggedright #1}}

